Convolutions and More as Einsum: A Tensor Network Perspective with Advances for Second-Order Methods

Despite their simple intuition, convolutions are more tedious to analyze than dense layers, which complicates the transfer of theoretical and algorithmic ideas to convolutions. We simplify convolutions by viewing them as tensor networks (TNs) that allow reasoning about the underlying tensor multiplications by drawing diagrams, manipulating them to perform function transformations like differentiation, and efficiently evaluating them with einsum. To demonstrate their simplicity and expressiveness, we derive diagrams of various autodiff operations and popular curvature approximations with full hyper-parameter support, batching, channel groups, and generalization to any convolution dimension. Further, we provide convolution-specific transformations based on the connectivity pattern which allow to simplify diagrams before evaluation. Finally, we probe performance. Our TN implementation accelerates a recently-proposed KFAC variant up to 4.5x while removing the standard implementation's memory overhead, and enables new hardware-efficient tensor dropout for approximate backpropagation.

==> exp/exp11_summarize_benchmark/fig/peakmems/kfac_reduce_factor_all_cpu.tex <==
% This file was created by tikzplotlib v0.9.7.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
axis line style={white!80!black},
log basis x={10},
tick pos=left,
xlabel={Auxiliary memory PT [MiB]},
xmin=0.478920515856782, xmax=4764.27163360104,
xmode=log,
ylabel={Auxiliary memory TN [MiB]},
ymin=0.513044481744355, ymax=1122.7248961758,
ymode=log,
zmystyle
]
\addplot [, color0, mark=*, mark size=3, mark options={solid}, only marks]
table {%
174.65234375 1
186.4609375 1
1 1
48.90625 1
61.82421875 1
292.93359375 1
286.68359375 1
70.9921875 31.7265625
142.8125 1
34.06640625 1
1 1
1 1
1 1
73.16015625 54.56640625
758.40625 86.66015625
758.7421875 84.359375
441.71875 52.0390625
178.05078125 1
84.6484375 1
127.84375 1
1 1
1 1
1 1
1 1
1 1
1 1
53.84765625 1
575.69921875 26.12109375
431.5 192.00390625
647.69140625 34.12109375
161.4921875 59.48046875
215.55859375 1
53.4921875 1
107.27734375 1
161.3359375 1
1 1
66.3203125 1
1 1
1150.97265625 576.0078125
575.21875 256.00390625
575.12890625 1
287.61328125 128.00390625
287.5625 1
144.00390625 1
144.00390625 1
3135.31640625 1
1567.84375 1
784.00390625 1
392.00390625 1
1 1
1 1
1 1
1 1
1 1
1 1
430.91796875 1
1 1
1 1
215.3984375 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
6.47265625 1
6.4140625 1
1 1
1 1
1 166.16015625
1 1
1 1
1 1
1 1
1 1
1 42.6640625
4.7578125 42.80859375
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
62.55859375 127.77734375
1 1
1 1
1 1
71.37890625 71.66015625
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
127.0703125 127.98828125
126.83984375 128
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
1 1
13.83203125 128
1 1
1 1
};
\addplot [, black]
table {%
0.727743912511554 0.727743912511554
791.497946732539 791.497946732539
};
\end{axis}

\end{tikzpicture}


==> latex-utilities/fdtexutils/checks/command_defined.tex <==
% IF-ELSE BASED ON WHETHER A COMMAND IS ALREADY DEFINED

\input{fdtexutils/checks/package_loaded}

% requirements
\assertPackageLoaded{etoolbox}

% If #1 is defined, expand to #2, else #3
\newcommand{\ifCommandDefinedElse}[3]{
  \ifdef{#1}{#2}{#3}
}


==> latex-utilities/fdtexutils/colors/pytorch.tex <==
% PYTORCH COLORS (from the new and old logos, https://pytorch.org/)

\input{fdtexutils/checks/package_loaded}
% requirements
\assertPackageLoaded{xcolor}

\definecolor{PTpurple}{RGB}{158, 82, 159}
\definecolor{PTorange}{RGB}{240, 87, 50}

==> latex-utilities/fdtexutils/colors/read_the_docs.tex <==
% COLORS FROM READTHEDOCS THEME

\input{fdtexutils/checks/package_loaded}
% requirements
\assertPackageLoaded{xcolor}

\definecolor{RTDBlue}{HTML}{2980b9}


==> latex-utilities/fdtexutils/colors/tuebingen_mpi.tex <==
% COLORS OF THE MAX PLANCK INSTITUTE FOR INTELLIGENT SYSTEMS IN TUEBINGEN.

\input{fdtexutils/checks/package_loaded}
% requirements
\assertPackageLoaded{xcolor}

% green color of Athena logo
\definecolor{MPIgreen}{RGB}{000, 125, 122}


==> latex-utilities/fdtexutils/colors/tuebingen_uni.tex <==
% CORPORATE DESIGN COLORS OF THE UNIVERSITY OF TUEBINGEN.

% They are documented at
% https://uni-tuebingen.de/en/einrichtungen/verwaltung/stabsstellen/hochschulkommunikation/service-fuer-beschaeftigte/corporate-design/basiselemente/farben/.
% Sadly, they can only be accessed via the intranet.

\input{fdtexutils/checks/package_loaded}
% requirements
\assertPackageLoaded{xcolor}

% PRIMARY COLORS
\definecolor{TUred}{RGB}{165, 30, 55}
\definecolor{TUgold}{RGB}{180, 160, 105}
\definecolor{TUanthrazit}{RGB}{50, 65, 75} % sometimes referred to as TUdark

% SECONDARY COLORS (groups are supposed to be used together)
% blues
\definecolor{TUdarkblue}{RGB}{65, 90, 140}
\definecolor{TUblue}{RGB}{0, 105, 170}
\definecolor{TUlightblue}{RGB}{80, 170, 200}

% greens
\definecolor{TUdarkgreen}{RGB}{50, 110, 30}
\definecolor{TUgreen}{RGB}{125, 165, 75}
\definecolor{TUlightgreen}{RGB}{130, 185, 160}

% reds/purples
\definecolor{TUlightpurple}{RGB}{180, 160, 150}
\definecolor{TUpurple}{RGB}{175, 110, 150}
\definecolor{TUlightred}{RGB}{200, 80, 60}

% oranges/browns
\definecolor{TUbrown}{RGB}{145, 105, 70}
\definecolor{TUorange}{RGB}{210, 150, 0}
\definecolor{TUlightbrown}{RGB}{215, 180, 105}

% UNOFFICIAL COLORS (from Philipp Hennig's beamer template)
\definecolor{TUgray}{RGB}{175, 179, 183}

==> latex-utilities/fdtexutils/fun/emojis.tex <==
% SOME FUN WITH TIKZ-MODIFIED LETTERS

\input{fdtexutils/checks/package_loaded}

% requirements
\assertPackageLoaded{tikz}

% Draw letter i with slightly smiling face as dot
\newcommand{\TikzLowercaseSlightlySmilingFaceI}{%
  {\tikz[baseline=-0.5ex]{% make aligned with text
      \node[draw=none,inner sep=0pt] (i) {\i};% letter i without dot
      \node[draw=none,inner sep=0pt] at ($(i.north)+(-0.088ex,0.412ex)$) {
        \resizebox{0.315ex}{!}{
          \TikzSlightlySmilingFace
        }
      };
      % for double-checking: overlay a read transparent i
      % \node[inner sep=0pt,draw=none,red,anchor=south,text opacity=0.5]
      % at (i.south) {i};
    }}}

% Draw a black slightly smiling face
\newcommand{\TikzSlightlySmilingFace}{\tikz{% https://tex.stackexchange.com/q/244759
    \draw[draw=none,fill=black] circle (2mm);
    \node[fill=white,circle,inner sep=0.5pt] (left eye) at (135:0.8mm) {};
    \node[fill=white,circle,inner sep=0.5pt] (right eye) at (45:0.8mm) {};
    \draw[white] (-145:0.9mm) arc (-120:-60:1.5mm);
  }}

==> sections/backlog.tex <==
\paragraph{Fusing convolutions:}
``It should be noted that a two step convolution operation can always to
combined into one'' (\url{https://iamaaditya.github.io/2016/03/one-by-one-convolution/})
Naive idea:
$\tW_2 \star \left( \tW_1 \star \tX \right) = \left( \tW_2 \star \tW_1 \right) \star \tX$

A simple example would be if we set kernel size to 1, stride to 1, padding to 0,
such that the output dimension does not change, i.e. $I = O$. In this case, we
have $\etPi_{:,:,k} = \mI_{I}$.

Like
\url{https://www.researchgate.net/publication/311754552_Fused-layer_CNN_accelerators}

Fusing with avg pooling after.

Higher-order AD functionality, such as multiplication by the second-order
derivative $\frac{\partial^2 \tY}{\partial \tX \partial \tW}$ for building up a
low-rank approximation of the Hessian~\cite{martens2012estimating}.

For instance, the XLA compiler~\cite{sabne2020xla} excludes convolution in the
list of fusible instructions~\cite{snider2023operator}.

These multi-linear operations are usually separated by non-linear activation
layers, which make it challenging to apply optimizations techniques specifically
developed for tensor contractions. In fact, many efforts in speeding up
computations focus on operator fusion. However, many computations arising in the
computation of higher-order information (like Hessian approximations or gradient
statistics) feature sub-computation graphs described by multi-linear tensor
operations, which can benefit from other optimization techniques. Here, we apply
these techniques to convolutions and investigate their potential to speed up
computations.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/conv4d.tex <==
Many popular machine learning libraries like PyTorch~\cite{paszke2019pytorch}
and TensorFlow~\cite{abadi2015tensorflow} only support convolutions on one- to
three-dimensional inputs\footnote{JAX~\cite{bradbury2018jax} supports
  convolutions of arbitrary dimension
  (\href{https://jax.readthedocs.io/en/latest/notebooks/convolutions.html\#basic-n-dimensional-convolution}{documentation}).}.
Many scientific applications require higher-dimensional convolutions, for
instance on four-dimensional inputs in confocal microscopy
reconstruction~\cite{page2020learning}, learning long-range spatio-temporal
interactions in video data, or object position estimation in OCT
volumes~\cite{bengs2020spatio-temporal}. To realize four-dimensional
convolution, those works used numerical tricks and implemented it by stacking
three-dimensional convolutions\footnote{We found numerous implementations of
  this
  approach:
  \href{https://github.com/msight-tech/research-v4d}{1},
  \href{https://github.com/pvjosue/pytorch_convNd}{2},
  \href{https://github.com/timothygebhard/pytorch-conv4d}{3} in PyTorch,
  and
  \href{https://github.com/funkey/conv4d}{4},
  \href{https://github.com/ngessert/4d\_deep\_learning}{5} in TensorFlow.}. The
tensor network formulation of convolution allows for a natural generalization to
higher-dimensional inputs~\cite{hayashi2019einconv} by adding contractions
with index pattern tensors along the additional axes.

We compare the performance of four-dimensional convolution via tensor networks
and via stacked three-dimensional convolutions for the LFMNet layer
of~\cite{page2020learning} in

\begin{table}[tbh]
  \centering
  \caption{Performance comparison of the four-dimensional convolution of
    LFMNet~\cite{page2020learning}. We compare the tensor network implementation
    with the approach based on stacked three-dimensional convolutions used
    by the original work. The input has batch size $128$, a single input channel, and
    spatial dimensions $(33,33,39,39)$. We compare convolutions with unit
    stride, padding $(1,1,0,0)$ and kernel size $(3,3,9,9)$ for different
    numbers of output channels (no bias).}
  \label{tab:performance-comparison-4d-convolution}
  \begin{tabular}{l}
    TODO
  \end{tabular}
\end{table}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

